Data-Driven Approach for Distribution Network Topology Detection

This paper proposes a data-driven approach to detect the switching actions and topology transitions in distribution networks. It is based on the real time analysis of time-series voltages measurements. The analysis approach draws on data from high-precision phasor measurement units ($\mu$PMUs or synchrophasors) for distribution networks. The key fact is that time-series measurement data taken from the distribution network has specific patterns representing state transitions such as topology changes. The proposed algorithm is based on comparison of actual voltage measurements with a library of signatures derived from the possible topologies simulation. The IEEE 33-bus model is used for the algorithm validation.

==> Conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper we propose a novel strategy for the monitoring and the identification of switches action in a distribution grid. It allows us, exploiting a voltage phasorial measurements, to understand both the time of the switches action and the new topology.
We deal also with the fast time scale load variation, of which we propose a model and validate it using real load data. Finally we show some simulations of the algorithm.

==> Placement.tex <==
\section{PMUs placement}
\label{sec:placement}
%
The first issue is the \emph{observability} problem, i.e. we have to find a criteria that tell us if, fixed the number of PMU to be deployed in the grid, there exist one or more way to dispose them in order to detect the topology change. Since our algorithm is basically based on the comparison between trend vectors and the library vectors, the trivial condition for the observability of the network is that each vector of the library is not proportional to any of the others. The former property is equivalent to the following condition.
%
\begin{lemma}
Given the set of nodes endowed with PMUs $\mathcal P$ let, with a slight abuse of notation, the juxtaposition of the library vectors be denoted by $\mathcal L_{\mathcal P}$. Then if 
%
\begin{equation}
[|\mathcal L_{\mathcal P}^* \mathcal L_{\mathcal P}|]_{uv} < 1, \forall u \neq v
\label{eq:lemm1_obsv}
\end{equation}
%
the switch that changes its status can be identified.
\label{lem:obsv1}
\end{lemma}
%
Notice that the element $[\mathcal L_{\mathcal P}^*\mathcal L_{\mathcal P}]_{uv}$ is simply the projection of $g_{[\sigma(t)]_{-u}}$ onto $g_{[\sigma(t)]_{-v}}$. If they are note purely proportional, trivially the magnitude of their inner product is smaller than one. 

Actually, condition \eqref{eq:lemm1_obsv} can be too much restrictive, if we assume to know the switches status before the topology change. In that case, in fact, we could require just that each vector of the \emph{particular} library is not proportional to any of the others. The former property is equivalent to the following condition.
%
\begin{lemma}
Let the switches state before the topology change be $\sigma(t)$, and let it be known. Then if 
%
\begin{equation}
[|\mathcal L_{\mathcal P,\sigma(t)}^* \mathcal L_{\mathcal P,\sigma(t)}|]_{uv} < 1, \forall u \neq v, \forall \sigma(t)
\label{eq:lemm2_obsv}
\end{equation}
%
each switch action can be identified.
\label{lem:obsv2}
\end{lemma}
%

Lemmas \ref{lem:obsv1} and \ref{lem:obsv2} can be used to infer, given the electrical grid, which is the minimun number of PMUs to be deployed in order to have observability. 

The second issue is to find an ``optimal'' placement. The notion of optimal is always relative to objective function to be maximized. 
%The paper main scope is to propose this novel approach for switches status, and thus we haven't already analyzed deeply the problem of optimal placement, neither how can it be stated as a formal optimization problem, that could eventually solved in an efficient way. 
However, here we propose a simply, even if onerous, strategy for placement, not necessary the best. 
After having found a minimal number of sensors and a place that guarantee the satisfaction of Lemma \ref{lem:obsv1}, we propose a greedy PMU placement procedure based on the sequential addition of one PMU at a time able to provide the best performance improvement, verified by Monte Carlo simulations. 
For every possible new place for PMU, we run num{\textunderscore}run Monte Carlo simulation, of length TSTOP. For each of them we choose , randomly, the initial $\sigma$, the switch $\ell$ that changes its status and the time $\tau$ of the action. The place for the new PMU that perform the minor number of errors is then chosen.
%

\begin{algorithm}
\caption{Greedy PMU placement}
    %
    \begin{algorithmic}[1]
      \Require $\mathcal P $ such that the network is observable, num{\textunderscore}run, TSTOP 
			\State min $\leftarrow \infty$
			\State minimizer $\leftarrow \emptyset$
				\For{every possible place $j \notin \mathcal P$}
					\State err $ \leftarrow 0$
					\For{$t = 1$ to num{\textunderscore}run}
						\State choose $\sigma \sim \mathcal U([0,1]^\noswitches)$
						\State choose $\ell \sim \mathcal U([0,\dots,\noswitches])$
						\State choose $\tau \sim \mathcal U([0,\text{TSTOP}])$
						\State run Monte Carlo simulations
						\State err = number of errors
						\If{err $\leq$ min} 
							\State $\min \leftarrow $ err
							\State minimizer $\leftarrow j$
						\EndIf
					\EndFor
				\EndFor
			\State $\mathcal P \leftarrow \mathcal P \cup \{\text{minimizer}\} $ 
    \end{algorithmic}
    %
\label{alg:greedy}
\end{algorithm}
%
